Can GPT-4 Identify Propaganda? Annotation and Detection of Propaganda Spans in News Articles

The use of propaganda has spiked on mainstream and social media, aiming to manipulate or mislead users. While efforts to automatically detect propaganda techniques in textual, visual, or multimodal content have increased, most of them primarily focus on English content. The majority of the recent initiatives targeting medium to low-resource languages produced relatively small annotated datasets, with a skewed distribution, posing challenges for the development of sophisticated propaganda detection models. To address this challenge, we carefully develop the largest propaganda dataset to date, ArPro, comprised of 8K paragraphs from newspaper articles, labeled at the text span level following a taxonomy of 23 propagandistic techniques. Furthermore, our work offers the first attempt to understand the performance of large language models (LLMs), using GPT-4, for fine-grained propaganda detection from text. Results showed that GPT-4's performance degrades as the task moves from simply classifying a paragraph as propagandistic or not, to the fine-grained task of detecting propaganda techniques and their manifestation in text. Compared to models fine-tuned on the dataset for propaganda detection at different classification granularities, GPT-4 is still far behind. Finally, we evaluate GPT-4 on a dataset consisting of six other languages for span detection, and results suggest that the model struggles with the task across languages. Our dataset and resources will be released to the community.

==> sections/task.tex <==
\section{Task Definition}
\label{sec:tasks}
The task of propaganda detection in text has been formulated covering different classification granularities. It ranged from modeling the problem as a binary classification task (propaganda vs. non-propaganda)~\cite{AAAI2019:proppy}, to a sequence tagging task where the aim is to extract spans of text containing persuasion techniques aiming to influence readers~\cite{EMNLP19DaSanMartino,piskorski2023news,piskorski2023semeval}.  Propaganda and persuasion are closely-related, as both aim at influencing readers and both employ persuasion strategies~\cite{jowett2018propaganda}. As previously done in literature, we use these terms interchangeably in this work. We model the task into four granularities, grouping those commonly-observed in literature as follows:
\begin{itemize}
    \item Propaganda text spans identification (Span): Given a text snippet, identify propaganda techniques it contains and text spans in which these techniques are being used. In our work, we adopt an existing two-tier taxonomy of six main categories, grouping 23 persuasion techniques~\cite{piskorski2023news}. That taxonomy represents the most comprehensive effort we identified aiming to model propaganda use in text over a variety of languages. 
    \item Propaganda techniques detection (Multilabel): Given a text snippet, identify propaganda techniques it contains from the 23 persuasion techniques.
    \item Coarse-grained propaganda detection (Coarse): Given a text snippet, detect the high-level categories of propaganda techniques it contains from the six categories.
    \item Binary propaganda detection (Binary): Given a text snippet, detect whether it uses any propaganda technique or not. 
\end{itemize}
